A Utility-Preserving Obfuscation Approach for YouTube Recommendations

Online content platforms optimize engagement by providing personalized recommendations to their users. These recommendation systems track and profile users to predict relevant content a user is likely interested in. While the personalized recommendations provide utility to users, the tracking and profiling that enables them poses a privacy issue because the platform might infer potentially sensitive user interests. There is increasing interest in building privacy-enhancing obfuscation approaches that do not rely on cooperation from online content platforms. However, existing obfuscation approaches primarily focus on enhancing privacy but at the same time they degrade the utility because obfuscation introduces unrelated recommendations. We design and implement De-Harpo, an obfuscation approach for YouTube's recommendation system that not only obfuscates a user's video watch history to protect privacy but then also denoises the video recommendations by YouTube to preserve their utility. In contrast to prior obfuscation approaches, De-Harpo adds a denoiser that makes use of a "secret" input (i.e., a user's actual watch history) as well as information that is also available to the adversarial recommendation system (i.e., obfuscated watch history and corresponding "noisy" recommendations). Our large-scale evaluation of De-Harpo shows that it outperforms the state-of-the-art by a factor of 2x in terms of preserving utility for the same level of privacy, while maintaining stealthiness and robustness to de-obfuscation.

==> docs/graveyard.tex <==
intro

Recommendation systems have been widely used to enhance the user web browsing experience by recommending items (e.g. videos, music, ads) based on a user's interests. 
%
YouTube, a video streaming site, is one of the most popular recommendation systems.
%
It receives an enormous influx of daily user activity and users have personalized YouTube accounts based on their interests. 
%
However, this raises privacy issues since modern recommendation systems, like YouTube, rely on users' personal data to provide accurate recommendations. 



%
To circumvent this privacy leakage in recommendation systems, researchers have proposed varieties of privacy-enhancing obfuscation approaches \cite{e02a5755350849eba1363e24b27d8ed2,URL_TRACKTHIS,Meng14,Degeling18,Kim18}.
However, they are limited in the fact that they focus on privacy only.

Moreover, obfuscation in recommendation systems is a tricky domain since users also want to maintain the utility of the recommendation system in order to get useful recommendations. Therefore, for recommendation systems, preserving utility alongside privacy is also imperative. Researchers have also proposed several mechanisms to balance this privacy-utility trade-off \cite{10.1145/3289600.3291026, zhang2021harpo, Huang17} but they are all limited in the fact that they achieve this trade-off by altering the input to the recommendation system, thus compromising on potential privacy gains.

In this paper, we propose \ToolX, a utility-preserving obfuscation approach for YouTube's recommendation system, which obfuscates a users' video watching history in order to enhance user privacy on YouTube, while preserving the user utility of using the recommendation system (i.e. receiving high-quality recommendations). To this end, \ToolX uses an \Obfuscator to inject obfuscation videos into YouTube users' video watch histories and a \Denoiser to remove recommended videos unrelated to users' actual interests. 

The \Obfuscator is a RL model that is trained to  insert YouTube videos in a users' watch history that will maximize the distortion in their interests being inferred by YouTube. The \Denoiser is a ML model that is trained to reproduce the original recommendations that would have been received in the absence of the \Obfuscator. This works because only \ToolX has information regarding the original non-obfuscated watching history, which is taken as the input of \Denoiser.

We evaluate \ToolX against the real-world YouTube recommendation system. Our evaluation results demonstrate that \ToolX can successfully increase the divergence of recommended video category distribution using the \Obfuscator, while reducing the utility loss caused by obfuscation significantly with the usage of \Denoiser.

Our main contributions are summarized as follows:
\begin{itemize}
\item We propose \ToolX, a utility-preserving obfuscation approach for YouTube's recommendation system. It uses an \Obfuscator to obfuscate users' video watching history and a \Denoiser to remove noise in video recommendations.
\item We design a surrogate model to replicate YouTube's recommendation system, such that we can train \ToolX offline effectively.
\item We demonstrate the effectiveness of \ToolX in both enhancing user privacy and preserving user utility against the real-world YouTube recommendation system .
\end{itemize}




---------


\subsection{Recommendation Systems}

Prior approaches for recommendation systems (e.g., matrix factorization \cite{mnih2007probabilistic,shan2010generalized,ma2008sorec,jamali2010matrix,ma2011recommender,tang2013exploiting,tang2016recommendations,yang2016social}, neural MF \cite{he2017neural,he2018outer,chen2020efficient,deng2016deep,wang2017item,zhao2017social,fan2018deep,fan2019deep}) to learn latent user-item relationships are not scalable because they rely on a fixed set of users and items.
%
To address this limitation, recent work has focused on embedding based recommendation systems that \hl{?how?} and thus can scale to a large and dynamic set of users and items \cite{?}.
%
YouTube, for example, deals with a large influx of videos and users everyday -- with more than 500 hours of new videos uploaded every minute \cite{?}. 
%
To this end, YouTube uses a scalable recommendation system that predicts the next watched videos by taking as input the embeddings of the past watched videos and other factors \cite{covington2016deep}.
%
Similar to YouTube's embedding based recommendation architecture, we design a surrogate model for YouTube's recommendation system that is designed to predict the recommended video category distribution, instead of making video-level recommendations. 
%
This design choice was made to (1) mitigate the impact of non-determinism in YouTube's recommendations and (2) alleviate the difficultly of making fine-grained video-level recommendations given incomplete set of videos available to us. 






%To this end, YouTube represents videos using embeddings and predicts the next watched videos by taking as input the embeddings of the past watched videos \cite{covington2016deep}.



In \cite{mnih2007probabilistic,shan2010generalized,ma2008sorec,jamali2010matrix,ma2011recommender,tang2013exploiting,tang2016recommendations,yang2016social}, matrix factorization (MF) has been used as the main technique for collaborative filtering in recommendation system, which projects the user and item vectors into a shared latent space and then use their inner product to model the preference of a user on an item. 
%
Later, to enhance the performance of MF-based recommendation algorithms, neural MF approaches have been proposed in \cite{he2017neural,he2018outer,chen2020efficient,deng2016deep,wang2017item,zhao2017social,fan2018deep,fan2019deep}, where deep neural networks (DNNs) are leveraged to learn the latent features of users and items and predict users' preferences on items. 
%
More recently, graph neural networks (GNNs) \cite{ying2018graph,monti2017geometric,wu2020diffnet++} have been used in recommendation systems. 
%
However, these approaches rely on a fixed set of users and items, which are not scalable. 
%
To address this problem, YouTube has proposed a scalable recommendation system based on deep learning, which represents videos using embeddings and predicts the next watched videos by taking as input the embeddings of the past watched videos \cite{covington2016deep}.
%
Our surrogate model is built on top of this architecture.
%
Different than the one used by YouTube, our surrogate model is designed to predict the recommended video category distribution of a given user persona, instead of making video-level recommendations.

\subsection{Privacy-Enhancing Obfuscation}
Prior work has proposed obfuscation approaches to enhance privacy of users in various online domains.   
%
However, a vast majority of prior obfuscation approaches are not designed to explicitly preserve the utility of the system while also enhancing privacy.
%

Firstly, we'll look at systems designed to throw off personalization for online ad targeting.
%
Initial work by Xing et al \cite{xing2013take} showed that attackers could easily perturb the personalized recommendations on YouTube, Amazon and Google.
%
Building from that, Meng et al \cite{Meng14} and Kim et al \cite{Kim18} developed ingenious ways to waste advertisers' ad budgets by creating polluting attacks and creating fake profiles respectively.
%
These showed that methods to alter online personas that can put off ad targeters were highly effective.

%
Moving to online profile obfuscation. TrackThis \cite{URL_TRACKTHIS} and AdNauseam \cite{e02a5755350849eba1363e24b27d8ed2} are great intros into methods to obfuscate the online profile of a user.
%
However, they suffer from not adapting to the user's online browsing profile.
%
\ToolX is adaptive as it interleaves the obfuscation videos according to the user's browsing history in a way that maximizes obfuscation.
%
Additionally, Degeling et al, \cite{Degeling18} designed and evaluated an obfuscation approach to “trick” a real-world user profiling system. 
%
They constructed user personas based on links posted on Reddit and showed how their obfuscation techniques threw off Oracle BlueKai's user profiling model. 
%
However, some obfuscation methods do try to tackle the problem of preserving utility. 
%
Beigi et al, \cite{10.1145/3289600.3291026} proposed to use greedy search and topic modeling to suitably obfuscate a users' browsing profile while also keeping utility in consideration.
%
Beiga et al, \cite{Biega17} assigned user requests to Mediator Accounts (MA) mimicking real users, such that (i) individual user profiles are scrambled across MAs to counter profiling, while (ii) coherent fragments of a user’s profile are kept intact in the MAs to keep user utility high. They relied on their user fragments in the mediator accounts to be coherent enough to preserve utility.
%
Finally, Zhang et al, \cite{zhang2021harpo} tried to preserve utility in their RL based obfuscation approach by cordoning off interest segments into "allowed" and "disallowed" segments in Personalized HARPO. Utility was preserved by receiving ads from the allowed segments. 
%
All of these methods aren't directly applicable to our domain of preserving utility in a Recommender System.
%

Another very common practice to preserve utility is to use Generative Adversarial Networks (GANs) in a privacy framework known as Generative Adversarial Privacy (GAP). 
%
This was introduced by Huang et al in Context-aware generative adversarial privacy \cite{Huang17}.
%
In this "GAP Loop", the privacy-utility tradeoff is maintained by a a \textit{privatizer} that obfuscates the input data, and an \textit{adversary} that tries to infer private information about the input data. 
%
They are jointly trained until an equilibrium state between the two is reached.
%
This mechanism is frequently used in privatizing mobile sensor data \cite{RavalMachanavajjhalaPan+2019+5+25}, \cite{Malekzadeh19}, \cite{Liu19}, camera sensory data in Autonmous Vehicles \cite{Xiong19} and in cloud based data compression \cite{Tseng20}.
%
\ToolX also was inspired by the "GAP loop" but we separately trained the RL-based Obfuscator and the LSTM-based Denoiser instead of jointly training them to reduce overheads. 
